A Hierarchical Subspace Model for Language-Attuned Acoustic Unit Discovery

In this work, we propose a hierarchical subspace model for acoustic unit discovery. In this approach, we frame the task as one of learning embeddings on a low-dimensional phonetic subspace, and simultaneously specify the subspace itself as an embedding on a hyper-subspace. We train the hyper-subspace on a set of transcribed languages and transfer it to the target language. In the target language, we infer both the language and unit embeddings in an unsupervised manner, and in so doing, we simultaneously learn a subspace of units specific to that language and the units that dwell on it. We conduct our experiments on TIMIT and two low-resource languages: Mboshi and Yoruba. Results show that our model outperforms major acoustic unit discovery techniques, both in terms of clustering quality and segmentation accuracy.

==> figures/hshmm_graph.tex <==
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
var/.style={circle, draw=black, minimum size=30pt},
obs/.style={circle, draw=black, fill=gray!80, thick, minimum size=30pt},
det/.style={rectangle, draw=black, minimum size=30pt}
]
\node[var] (hyper_subspace) {$\mathcal{M}$};
\node[det] (subspace) [right=of hyper_subspace] {$\Matrix{W}^\lambda, \Matrix{b}^\lambda$};
\node[var] (lang_emb) [below=of subspace] {$\Matrix{\alpha}^\lambda$};
\node[det] (param) [right=of subspace] {$\Matrix{\eta}^{\lambda, u}$};
\node[var] (unit_emb) [below=of param] {$\Matrix{e}^{\lambda,u}$};
\node[obs] (data) [right=of param] {$\Matrix{x}_n$};
\node[var] (current) [below=of data] {$z_n$};
% \node[var] (prev) [left=of current] {$z_{n-1}$};

\draw[black, ->, thick, dashed] (hyper_subspace.east) -- (subspace.west);
\draw[black, ->, thick, dashed] (lang_emb.north) -- (subspace.south);
\draw[black, ->, thick, dashed] (subspace.east) -- (param.west);
\draw[black, ->, thick, dashed] (unit_emb.north) -- (param.south);
\draw[black, ->] (param.east) -- (data.west);
\draw[black, ->] (current.north) -- (data.south);
% \draw[black, ->] (prev.east) -- (current.west);
% \draw[rounded corners] (-0.8, -3) rectangle (0.8, 0.8) {};
\draw[rounded corners] (1.2, -3) rectangle (3.2, 0.8) {};
\draw[rounded corners] (3.6, -3) rectangle (5.2, 0.8) {};
\draw[rounded corners] (5.6, -3) rectangle (7.2, 0.8) {};
\node at (2.6, -2.8) [shape=rectangle, rounded corners, text=black] {$1\dots L$};
\node at (4.6, -2.8) [shape=rectangle, rounded corners, text=black] {$1\dots U^\lambda$};
\node at (6.6, -2.8) [shape=rectangle, rounded corners, text=black] {$1\dots N^\lambda$};

% \node[shape=rectangle, rounded corners, inner sep=0pt, draw=black, text=black, text height=2.2cm] {test};

% \draw[rounded corners] (1.4, -5.5) rectangle (3, -1) {};
% \draw[rounded corners] (3.2, -5.5) rectangle (7, -1) {};

% \draw[rounded corners] (-1, -5.5) rectangle (1.2, -1) {};
% \draw[rounded corners] (1.4, -5.5) rectangle (3, -1) {};
% \draw[rounded corners] (3.2, -5.5) rectangle (7, -1) {};


% \node[var] (current) [above=of data] {$z$_{n-1}};

% \draw[black, thick] (0,-0.5) circle (0.5) node[anchor=center]{$\mathcal{M}$};
% \draw[black, thick] (0,2.5) circle (0.5) node[anchor=center]{$\Matrix{\alpha}^\lambda$};
% \draw[black, thick] (-0.5 , 0.5) rectangle (0.5, 1.5);
% \draw[black, ->, dashed] (0, 0) -- (0,0.5);
% \draw[black, ->, dashed] (0, 2) -- (0,1.5);
% \node[squarednode]      (maintopic)                              {2};
% \node[observedvarnode] (x) {X};
% \node[detvarnode] (W) [right=of x] {W, b};
\end{tikzpicture}

==> inputfiles/acknowledgment.tex <==
We have a few people we would like to thank from the group and especially from the Machine learning group. Alas, we have little space and we must acknowledge the Money A. Grant Foundation and the Government Fund Big Time Money Money 811911001 for giving us money to live a researcher's glorious life above minimum wage. Thanks a lot. The machine learning group guys really should have given us more money to get their names here.
